New Technologies for Discovery

For the field of high energy physics to continue to have a bright future, priority within the field must be given to investments in the development of both evolutionary and transformational detector development that is coordinated across the national laboratories and with the university community, international partners and other disciplines. While the fundamental science questions addressed by high energy physics have never been more compelling, there is acute awareness of the challenging budgetary and technical constraints when scaling current technologies. Furthermore, many technologies are reaching their sensitivity limit and new approaches need to be developed to overcome the currently irreducible technological challenges. This situation is unfolding against a backdrop of declining funding for instrumentation, both at the national laboratories and in particular at the universities. This trend has to be reversed for the country to continue to play a leadership role in particle physics, especially in this most promising era of imminent new discoveries that could finally break the hugely successful, but limited, Standard Model of fundamental particle interactions. In this challenging environment it is essential that the community invest anew in instrumentation and optimize the use of the available resources to develop new innovative, cost-effective instrumentation, as this is our best hope to successfully accomplish the mission of high energy physics. This report summarizes the current status of instrumentation for high energy physics, the challenges and needs of future experiments and indicates high priority research areas.

==> Challenges.tex <==
\section{Challenges}
\label{s.challenge} 

\subsection{Key Challenge I: Quantum Sensors}  

Quantum sensors based on superconducting detector and readout technology are at the core of a diverse
set of HEP experiments and have a broad range of potential applications, including quantum computing,
the defense industry, and astronomy. A compelling aspect of HEP quantum sensor R\&D is the interplay
between improvements in detector technology and leadership in HEP science. HEP science provides a
well-defined framework for quantum sensor development while improvements in quantum technology directly
advance the frontier of HEP science. In many cases, HEP innovation can then be exported to other
non-HEP applications. This interplay and impact motivates a strategic investment in superconducting
detector R\&D within the context of HEP applications.
The focus of this investment should be on sensitivity and scale.

The exceptional sensitivity of superconducting detectors enables exploration beyond the limits
of silicon technology. As such, they are the favored technology for probing particle physics
associated with low-energy threshold experiments, including: dark matter searches
(e.g., low-mass WIMPs and axions), and neutrino studies (e.g., double-beta-decay and coherent
neutrino scattering). Outside of HEP, similar detectors and technology can be used to study
quantum systems, and can form the basis of quantum computers. The first goal of the quantum
sensor challenge is to increase the sensitivity of superconducting technology through
developing ultra-low threshold ($<20$~mK) dark matter detectors and sub-quantum limited amplifiers for axion and axion-like particle searches.  

The scalability of superconducting detectors enables the benefits of superconducting sensitivity at substantive detector masses and channel counts.  The second goal of the quantum sensor challenge is to realize systems with densities comparable to semi-conductor devices.
Deploying ``megapixel'' scale experiments will advance next-generation cosmic microwave background (CMB) studies with impact on other calorimetric applications, including beta-decay and X-ray spectroscopy.
The same technology enables cameras from the optical to the mm-wave that have been proposed for next-generation dark energy experiments, sub-mm astronomy, homeland security, and nuclear non-proliferation. To achieve this goal, the field requires high-volume detector testing, fabrication, and production and increased multiplexing density of detector readouts.
This goal is best achieved through developing large-scale technology for mm-wave bolometers for CMB experiments.


The technological goals for the quantum sensors challenge can be encompassed in the following “10-100-1000” rubric:
\begin{itemize}
\item Over 10-times reduction in noise and threshold
\item Over 100-times increase in fabrication throughput
\item Over 1000-times increase in signal bandwidth and readout density
\end{itemize}

\subsection{Key Challenge II: Photo Sensors}

Photo Sensors are integral to almost every large detector in HEP, from dark matter
and neutrino experiments to collider detectors at the LHC. In addition,
Photo Sensors are widely used outside of HEP – thus advances made in this realm
tend to have direct and immediate uses in medicine, industry, and other scientific
fields. It is often the case that HEP catalyzes industrial R\&D for the development
of new instruments, providing expertise and testing facilities in addition to an
initial market to help defray R\&D costs.

Photo Sensor performance is characterized by:
\begin{itemize}
\item timing resolution
\item spectral sensitivity
\item efficiency
\item radio-purity
\item cost.
\end{itemize}
All these characteristics are being actively improved upon in order to increase sensitivity of future experiments,
but the first two are especially relevant.

Timing resolution: In many new detectors, fast timing is critical to improve sensitivity. This is due to the fact that the uncertainly in time translates directly into uncertainty in event vertex and track reconstruction.  New fast Micro-Channel Plates (MCPs) have achieved single photoelectron time jitter of 50-60 picoseconds. This is more than an order of magnitude better than current Photo-Multiplier Tubes (PMTs). Development of mass produced inexpensive MCPs is seen as the highest priority development in this area, as it opens the possibility to do new experiments that are not currently possible with existing technology. For example, it would be possible to build large hybrid neutrino detectors that combine tracking with low threshold and excellent energy resolution and particle identification. It would also be possible to operate fast photo-sensors in the high magnetic field environment of the LHC. 

Spectral Sensitivity: Cryogenic liquid noble gas detectors are coming into widespread use in HEP due to their excellent tracking and particle identification capabilities using both ionization drift and scintillation light. The scintillation capability is used to add timing to the relativity slow ionization measurements in order to allow operation in high rate environments such as the LHC and underground neutrino detectors that desire low thresholds. Unfortunately, spectral sensitivity of PMTs is poorly matched to the hard ultraviolet emission of argon and xenon, the two most widely used and available noble gasses and liquids. Researchers in industry are working on the development of silicon-based devices specifically for use in the hard ultraviolet.  This development is critical to improving the performance future cryogenic detectors.

Efficiency: The quantum efficiency of photocathodes remains well below 50\% and
the photo-detection efficiency of MCP-based detectors is around 70\%.
Through the development of new photocathode materials and modern detector
fabrication processes, large gains can be achieved through targeted R\&D. 

Radio-purity: In many low background detectors photodetectors play a crucial role in the rejection of background. These experiments carefully avoid any source of radio-impurities in the environment. The detectors themselves thus have to be very radio-pure. Significant improvements in the radio-purity of photodetectors would be very beneficial.  

Cost: The scale of particle physics detectors is often prohibitive to the deployment of photodetectors on a large scale. Large-area, cost-effective photodetectors could be a disruptive technology for many fields of science. 

The technological goals for photodetectors can be captured in the rubric ``SSERC Photodetectors''. 


\subsection{Key Challenge III: Dead-timeless Trigger and Data Acquisition Systems}

Future HEP accelerators will produce luminosities that will challenge today’s TDAQ designs and implementations. This is already becoming apparent with the highly successful Run 2 of the LHC. The HL-LHC will have luminosities around $7.5\times10^{34}$, and there are plans for an FCC capable of $3\times10^{35}$. The field of particle physics needs to develop new trigger and data acquisition technologies to be able to cope with extremely large instantaneous data volumes, to optimally mine the data collected, and to alleviate the demands on offline resources. A key challenge to demonstrate the individual technologies needed in a realistic environment would be a first step towards developing a complete system.

Compared to the present LHC detectors, which are today’s state of the art, a new paradigm has to be created. This could take shape in different ways, but some of the hurdles to overcome are: 
\begin{itemize}
  \item For the ATLAS and CMS detectors, the Level 1 accept rate will need to increase by an order of magnitude, to about 1 MHz, requiring a higher readout bandwidth of higher granularity detectors. In addition, the data volume used by the Level-1 trigger to make its decision at 40 MHz will greatly increase with higher granularity calorimeter and muon information, and tracking data (CMS).
\item An important challenge for this system is to extract the data at high bandwidth from the tracking detectors without adding a prohibitive burden of material due to the large number of fiber drivers and the power and cooling they would need. Hermetic detectors, such as CMS and ATLAS provide no path outside of the active region for the data and trigger fibers and drivers, which must survive in a harsh radiation and magnetic field environment.
\item 	Non-hermetic detectors such as LHCb plan to operate without a hardware Level-1 trigger, instead absorbing a large increase in data volume directly into software-based triggers running on next generation CPUs and GPUs, which by necessity must be some distance from the detector and its radiation and magnetic field environment.
\item 	In either case, High-level Trigger and beyond would have to process at least 10 times as much data. 
\item 	The overlap of detector front-end signals from different collisions and different beam crossings will increase by an order of magnitude, requiring more information (such as the z-vertex from tracking data and potential precise timing information) and much more sophisticated algorithms to separate them. 
\end{itemize}
Potential research directions could include: 
\begin{itemize}
\item 	Low-power and low mass technologies for deep buffers for a low deadtime system.  At Level 1, the minimum depth is the decision time divided by the beam crossing time (about 20 for the Tevatron and 100 for the LHC) plus the number of Level 2 buffers.  Typically, the required number of Level 2 buffers has been set using Poisson statistics and an acceptable level of dead-time, implemented with rules that prevent buffer overflow. Buffers located on tracking detectors would need low power and mass to avoid excessive material. Any buffers located in the experimental area would need radiation and magnetic field tolerance.
\item 	High bandwidth, low-power and low-mass fiber optics drivers that can function in a radiation and magnetic field environment in order to extract trigger and readout data from tracking detectors.
\item   Wireless data transmission and power distribution to reduce cables and material in the detector.
\item 	Technologies to extract, process and integrate fast timing information to provide an additional handle to reduce pileup of data from spatially and temporally proximate collisions.
\item 	Closer integration of embedded systems and programmable logic (e.g. FPGAs) with high bandwidth network integration to provide fast configuration, monitoring and control of the very large amounts of programmable logic required by the more complex Leve1-1 trigger.
\item 	Level-1 Triggers more closely integrated with Level 2 processors, thereby reducing the network between Level 1 and Level 2: when there is a Level 1 accept, the data is already in Level 2.
\item 	Use of heterogeneous processing combining CPUs, GPUs and other architectures to provide the large increase in processing power required for the software triggers, as well as the software technologies to exploit the new generation of processors.
\item 	Co-locate supercomputers at the experiment or embed them in the online framework to allow them to provide the computation for software-level triggering.  Total computation will most likely not prove to be a limitation, rather it is the networking in getting data into the supercomputer to begin with, and (if necessary) moving the data from node to node.
\end{itemize}
  
The final design might have applications beyond particle physics. The proposed Electron Ion Collider
could use this, in particular for the higher luminosity design.  Some of the new x-ray science
cameras might want to use this.  Their data volumes are smaller, but they still have a need for speed.

The technological goals for next generation trigger and data acquisition systems can be captured under the rubric “The Big Data Gulp”. 


\subsection{Key Challenge IV: Near Zero Silicon Detectors}

Vertex and tracking detectors require ultimate precision while at the same time insisting on near zero material budget, dead-time and power consumption, all this for radiation hard technologies. CMOS MAPS sensors have several advantages over traditional heterogeneous technologies with separate sensors and readout ASICs. The built-in amplifiers allow a reduction in signal, and therefore sensor thickness. Small feature size technologies make a fine readout pitch possible. The sensor periphery can accommodate a digital circuit for fast data readout and processing in-situ. The data can be serialized for readout, which drastically reduces the interconnect requirements. Instead of bump-bonding or wire-bonding every channel on a sensor, just a few wire-bonds for the data bus connection are sufficient. Furthermore, the CMOS devices are made at standard commercial foundries and therefore can be produced quickly and inexpensively. The integrated nature of the sensors and reduction in the number of interconnects facilitate a large tracker construction in a very short time at significantly reduced cost compared to today’s trackers. 

A key challenge for CMOS MAPS is to develop 50~$\mu$m thick devices with better than 5~$\mu$m position resolution that are radiation tolerant to $10^{16}$ n$_{eq}$/cm$^2$. An additional requirement is fully efficient readout at 25~ns bunch crossing time with up to 100 particles per sensor in a technology that enables construction of a 200~m$^2$ tracker in less than a year.

\subsection{Key Challenge V: Breaking the Picosecond Time Barrier}

High resolution timing information is a powerful discriminant in many experiments. In the context of
the LHC experiments, timing will provide a powerful handle to address pile-up. Particle identification
is also aided by timing information up to high momenta. Timing signals enable vertex reconstruction
in neutrino interactions and dark matter experiments. Having channel-by-channel timing information
available with sub-10 picosecond resolution would be disruptive. The technological challenges to
achieve this level of precision are formidable. Without specifying the technology, achieving
pico-second timing at the system level is a key challenge for the field and will be referred
to here as SPS detectors, for Sub Pico-Second detectors.  

\subsection{Key Challenge VI: Realtime Machine Learning for Particle Physics Trigger Systems}  

Bringing the modern algorithmic advances from the field of machine learning from offline applications to online operations and trigger systems is one of the major challenges. There are already examples of relatively simple machine learning algorithms implemented at both the hardware and software trigger levels of several experiments at the energy and intensity frontiers. However, more powerful algorithms based on deep learning have become the state-of-the art in a number of areas and applications, and bringing them to the trigger decision-making logic, including implementation on FPGAs and other accelerators that allow for the necessary trigger latency requirements, is one of the major challenges and also opportunities that the high-energy physics community today should exploit in the next several years. %Currently, there are research and development efforts in this direction that target both present and future experiments.  

